Testing Lorentz Invariance with Neutrinos

The search for a theory that unifies general relativity and quantum theory has focused attention on models of physics at the Planck scale. One possible consequence of models such as string theory may be that Lorentz invariance is not an exact symmetry of nature. We discuss here some possible experimental and observational tests of Lorentz invariance involving neutrino physics and astrophysics.

==> footmisc-code.tex <==
% this will typeset documentation + code

\AtBeginDocument{\AlsoImplementation}
\input{footmisc.dtx}

